Design Considerations for Low Power Internet Protocols

Over the past 10 years, low-power wireless networks have transitioned to supporting IPv6 connectivity through 6LoWPAN, a set of standards which specify how to aggressively compress IPv6 packets over low-power wireless links such as 802.15.4. We find that different low-power IPv6 stacks are unable to communicate using 6LoWPAN, and therefore IP, due to design tradeoffs between code size and energy efficiency. We argue that applying traditional protocol design principles to low-power networks is responsible for these failures, in part because receivers must accommodate a wide range of senders. Based on these findings, we propose three design principles for Internet protocols on low-power networks. These principles are based around the importance of providing flexible tradeoffs between code size and energy efficiency. We apply these principles to 6LoWPAN and show that the resulting design of the protocol provides developers a wide range of tradeoff points while allowing implementations with different choices to seamlessly communicate.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> code_size_table.tex <==
\begin{table*}[t]
\caption{6LoWPAN Stack Code Size for 6 open source stacks. The code size varies
by over a factor of 4, in part due to different feature sets. In some cases,
the size of the 6LoWPAN implementation is larger than the IPv6 stack. TinyOS's
whole-program optimization model precluded separating out subcomponents
of its implementation.
}\label{tab:b}
\begin{tabular}{lrrrrr}
\toprule
\bf{Stack}                              & \multicolumn{5}{c}{ \bf{Code Size Measurements (kB)} }          \\
\hline
                                        & \multicolumn{4}{|c|}{ \bf{6LoWPAN} }          & \\

	         & \multicolumn{1}{|r}{\bf{Compression}} & \bf{Fragmentation} & \bf{Mesh/Broadcast Headers} & \multicolumn{1}{c|}{\bf{Full}} & \bf{IP stack (L3 +)}      \\
\hline
Contiki      & 6.0       & 3.3    & N/A   & 11.3  & 26.2    \\
ContikiNG    & 3.4       & 1.9    & N/A   & 6.2   & TODO    \\
OpenThread   & 4.1-20.0  & 1.3    & 4.5   & 26.4  & 15.9    \\
Riot         & >4.7      & 1.5    & N/A   & 7.5   & 23.5    \\
Arm Mbed     & 18.0      & 3.1    & 1.3   & 22.1  & 23.9    \\
TinyOS       & -- --     & -- --  & 0.6   & 16.2  & 21.1    \\
\bottomrule 
\multicolumn{6}{l} * TinyOS inlines compression code into fragmentation code, and does not completely implement the mesh header \\
\end{tabular}
\end{table*}

%These values are for IP stacks including transport layer code but excluding things like
% security, routing, app layer (coap), and exluding link layer/radio driver code for some stacks.


==> impl.tex <==
\label{s:impl}
\begin{quote}
\it{"Every bit transmitted brings a sensor node one moment closer to death"}
  \begin{flushright}
    \tiny{---Greg Pottie~\cite{pottie}}
  \end{flushright}
\end{quote}

The 6LoWPAN specification was created with a clear goal---to allow for IPv6
connectivity over a link-layer with an order of magnitude smaller frame sizes
than Ethernet. Unfortunately, fragmented IPv6 on its own requires header
overhead much greater than typical wireless protocols designed for low power
devices. As a result, the specification places an extreme focus on minimizing
protocol overhead and, thus, radio utilization.

The primary problem with 6LoWPAN is that this focus was taken too far. This
focus has resulted in complex implementations that require significant processor
resources. In order for devices to interoperate, they must be able to parse any
valid received 6LoWPAN packet that might be sent by others.

In practice, as section~\ref{s:interop} shows, many 6LoWPAN implementation do
not implement the entire specification and, therefore, are not interoperable.
We argue that this is not a result of poor software design, but rather
{\it{intentional}} choices to implement different subsets of the specification
that favor limited RAM and code size, security concerns, and minimizing
engineering effort.

In fact, in some cases even these incomplete 6LoWPAN implementations systems are
too resource intensive for some devices. As a result, several implementations
allow the developer to remove portions of the 6LoWPAN stack during compilation.
Even when implementations use overlapping portions of the specification, additional
interoperability conflicts arise from different choices of memory bounds for
decompression.

\subsection{Processor Resources}

\input{code_size_table.tex}

%\subsubsection{ROM/RAM Assumptions}
%
%When the 6LoWPAN specification was designed, some consideration was given to the 
%fact that it would be implemented on low power microncontrollers with limited
%code space and RAM. In fact, "The 6LoWPAN Architecutre" ~\cite{Mulligan}, the paper 
%published by the IETF 6LoWPAN Working Group in 2007, contains a section titled
%"6LoWPAN - Not too big", which argues that 6LoWPAN requires code size comparable
%to other low power networking stacks such as Zigbee and Zensys. In fact, that paper
%claims that a fully functional 6LoWPAN implementation requires only 22 kB of code
%space and 4 KB of RAM for the entire 6LoWPAN/IPv6 stack . This estimation, and
%comparison to popular contemporary
%networking stacks, seem to serve as the primary justification that 6LoWPAN
%does not have problems related to code size/RAM. This assumption
%seems to have held since 2007, and subsequent amendments to the specification
%such as RFC 6282 and RFC 6775 do not appear overly concerned with affects on code
%size or RAM requirements. Unfortunately, these amendments have a significant 
%impact on the original estimates made. Further, this initial estimate understates
%the true code size and RAM requirements of a full 6LoWPAN stack by not accounting
%for the code size and RAM required to implement the rest of an IP stack, including
%transport layer code (TCP/UDP/ICMP) and code allowing these 
%devices to be managed within IP networks.
%
%In order to accurately gauge the impact of RAM/ROM limitations, we need
%a more complete and up-to-date picture of the code size and memory requirements
%of 6LoWPAN. "Implementation and Evaluation of the Enhanced Header Compression
%(IPHC) for 6LoWPAN" provides a more up to date estimate, noting that for one
%simple app on TinyOS using the updated header compression specified in RFC 6282
%increased ROM usage by 564 bytes. The authors note "This reflects the increased
%complexity of the compression algorithm.
%Mainly, the use of context based compression makes memory performance worse." 
%Unfortunately, it is difficult to determine exactly how much of RFC 6282 was
%implemented when this analysis was performed, as links to the code used for testing
%no longer work, and little description is provided regarding the example 
%application used to test memory requirements. To obtain a more up-to-date, 
%complete, and all-encompassing estimate of the code size requirements of 
%6LoWPAN, we measured the code size required for 6LoWPAN on each of the stacks
%analyzed in Section ~\ref{s:interop}. 

Evidence that developers of these 6LoWPAN stacks
were concerned about 6LoWPAN's consumption of processor resources is baked into
the design of each.
One of the primary indicators that
each implementation was concerned with code size is the prevalence of options to
compile limited subsets of the 6LoWPAN stack. For example, Contiki defines the
SICSLOWPAN\_CONF\_COMPRESSION compilation flag, which can be set to force all
Contiki packets (sent and received!) to be processed as uncompressed IPv6. Riot
presents extensive compilation options for 6LoWPAN, allowing for the exclusion of
all IPHC compression, the exclusion of context based compression alone, the
exclusion of fragmentation, the exclusion of ND, and the exclusion of next header compression.
The Mbed stack allows users to exclude 
elements of the IPv6 stack such as security features, routing specific features,
link-layer features, and more. Further, Mbed defines macros which can be
used to save RAM at the expense of flash, or vice-versa. TinyOS by default
removes all code in a stack that is not being used by an application, and 
we observed this at work by compiling different 6LoWPAN application binaries.

Table~\ref{tab:b} shows the code size overhead of each of the five
implementations broken into independent overheads for compression,
fragmentation, mesh and broadcast headers, as well as totals for 6LoWPAN and the
entire networking stack including physical layer drivers, IPv6, UDP, ICMP, etc.
The commit hash of each stack that was examined is contained in Table~\ref{tab:c}.

We estimate these values using two methods. We used existing options provided by
the Contiki and Riot build systems to remove particular 6LoWPAN functionality at
compile-time. For OpenThread, TinyOS, and Mbed, which do not have such options, we
manually analyzed binary build products using the \texttt{readelf} utility from
the GCC toolchain to isolate functions associated with each aspect of 6LoWPAN.

These results likely overestimate the overhead of fragmentation and
underestimate the overhead of certain kinds of compression since some of the
complexity of compression is born on the fragmentation logic. Moreover, for
OpenThread and Arm Mbed, where we had to examine binaries manually, we expect
the results underestimate the overhead of all 6LoWPAN components since we
only counted procedures which unambiguously implemented particular
functionality, though some of the complexity is implemented in other portions of
the stack. In summary:

%% What should the reader take away from these results, as a bullet list for
%% now
\begin{itemize}
    \item 6LoWPAN stack devolopers were concerned with 
        processor resource requirements of the protocol.
	\item Fragmentation, the only portion of 6LoWPAN that's strictly
		\emph{necessary} for sending IPv6 packets, consumes
		significantly less ROM than compression.
	\item Implementations with more complete adherence to compression
		specification consume more code for compression
	\item Mesh and broadcast headers are relatively expensive given that few
    	real-world applications use them
\end{itemize}

\subsection{COAP}

TODO


